Wormhole MAML: Meta-Learning in Glued Parameter Space

In this paper, we introduce a novel variation of model-agnostic meta-learning, where an extra multiplicative parameter is introduced in the inner-loop adaptation. Our variation creates a shortcut in the parameter space for the inner-loop adaptation and increases model expressivity in a highly controllable manner. We show both theoretically and numerically that our variation alleviates the problem of conflicting gradients and improves training dynamics. We conduct experiments on 3 distinctive problems, including a toy classification problem for threshold comparison, a regression problem for wavelet transform, and a classification problem on MNIST. We also discuss ways to generalize our method to a broader class of problems.

==> Algorithms/maml.tex <==
\begin{algorithm}[H]
\Require{$p(\mathcal{T})$: distribution over tasks}
\Require{$\alpha, \beta$: step size hyper-parameters}
Randomly initialize $\theta$\;
\While{not done}{
    Sample batch of tasks $\mathcal{T}_i \sim p(\mathcal{T})$\;
    \For{all $\mathcal{T}_i$}{
        Evaluate $\nabla_\theta \mathcal{L}_{\mathcal{T}_i}(\theta)$ with respect to $K$ examples\;
        Compute adapted parameters with gradient descent: $\phi_i \leftarrow \theta - \alpha \nabla_\theta \mathcal{L}_{\mathcal{T}_i}(\theta)$\;
    }
    Update $\theta \leftarrow \theta - \beta \nabla_\theta \sum_{\mathcal{T}_i \sim p(\mathcal{T})} \mathcal{L}_{\mathcal{T}_i}(\phi_i)$\;
}
\caption{Model-Agnostic Meta Learning}\label{alg:maml}
\end{algorithm}

==> Figures/loss_mnist.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{Figures/loss_mnist1.pdf}
\end{center}
\caption{\textbf{Loss curve analysis on the MNIST task.} (a) The training process is rather unstable without adapting to the wormhole parameter. (b) Learning wormhole parameter helps with training stability.}
\label{fig:loss_mnist}
\end{figure}

==> Sections/6_Contributions.tex <==
\section{Team Contributions}

The breakdown of the contributions of individual team members is as follows:

\begin{itemize}
    \item Beicheng: (1) Mathematical formulation for Wormhole MAML (2) Method analysis and characterization (3) MNIST dataset experiments (4) Poster and final report
    \item Yuan: (1) Framework implementation (2) Avg-threshold experiments (3) Wavelet transform experiments (4) Poster and final report
    \item Tracy: (1) Framework implementation (2) Avg-threshold experiments (3) MNIST dataset experiments (4) Poster and final report
\end{itemize}
